Acceleration via Symplectic Discretization of High-Resolution Differential Equations

We study first-order optimization methods obtained by discretizing ordinary differential equations (ODEs) corresponding to Nesterov's accelerated gradient methods (NAGs) and Polyak's heavy-ball method. We consider three discretization schemes: an explicit Euler scheme, an implicit Euler scheme, and a symplectic scheme. We show that the optimization algorithm generated by applying the symplectic scheme to a high-resolution ODE proposed by Shi et al. [2018] achieves an accelerated rate for minimizing smooth strongly convex functions. On the other hand, the resulting algorithm either fails to achieve acceleration or is impractical when the scheme is implicit, the ODE is low-resolution, or the scheme is explicit.

==> gradient_norm.tex <==
As a warm-up, we revisit gradient descent for smooth convex functions, highlighting the ODE-based approach and the importance of Lyapunov functions in proofs. Our finding is the following theorem.
\begin{thm}
	\label{thm: grad_descent_convex2}
	Let $f \in \mathcal{F}_{L}^{1}(\mathbb{R}^n)$.
	Taking step size $s =  1/L$, the iterates $\{x_{k}\}_{k = 0}^{\infty}$ generated by gradient descent~\eqref{eqn:gd} satisfy 
%	\begin{equation}
%	\label{eqn: gradient_descent_convex_2}
%	\left\{ \begin{aligned}
%	& f(x_{k}) - f(x^{\star})                                                  \leq     \frac{ \left\| x_{0} - x^{\star} \right\|^{2} }{2ks} \\
%	& \min_{0 \leq i \leq k}\left\| \nabla f(x_i) \right\|^{2}     \leq     \frac{ 2\left\| x_{0} - x^{\star} \right\|^{2} }{s^2(k + 1)(k + 2)}
%	\end{aligned} \right.
%	\end{equation}
%	In addition, if the step size is set $s = 1/L$, then
	\begin{equation}
	\label{eqn: gradient_descent_convex_21x}
	\sum_{i = 0}^{\infty} (i + 1)\left\| \nabla f(x_i) \right\|^{2}     \leq   L^2 \left\| x_{0} - x^{\star} \right\|^{2}.
	\end{equation}
\end{thm}
This theorem directly implies that
\[
\min_{0 \le i \le k} \|\nabla f(x_i)\|^2 \le \frac{\sum_{i=0}^k (i+1)\|\nabla f(x_i)\|^2}{\sum_{i=0}^k (i+1)} = O\left( \frac{L^2 \|x_0 - x^\star\|^2}{k^2} \right),
\]
which is known in the literature \citep{nesterov2012make}. However, our result is stronger in the sense that the $O(L^2/k^2)$ rate does not imply \eqref{eqn: gradient_descent_convex_21x}.
%than the  rate since 
%While the $O(L/k)$ convergence rate for the function value is classical, the $O(L^2/k^2)$ convergence rate for the squared gradient norm cannot be obtained using classical analysis of \gd.
%\bin{A two-step proof, combined with standard convex inequality and function value bound, is first shown in~\citep{nesterov2012make}}
%\bin{Remark: The second inequality is stronger than the rate $O(L^{2}/k^{2})$. Some similar results are in~\cite{attouch2016rate, shi2018understanding}.  If the limit exists 
%\[
%\lim_{k \rightarrow \infty} k^{2} \left\| \nabla f(x_{k}) \right\|^{2},
%\]
%then the rate of the gradient norm minimization is actually 
%\[
%\left\| \nabla f(x_k) \right\|^{2} \leq o\left( \frac{L^{2} \left\| x_0 - x^\star \right\|^{2}}{k^{2}} \right)
%\]
%}

To obtain this result, we use a Lyapunov function that is different from the standard analysis of gradient descent, which uses the Lyapunov function $\mathcal{E}(k) \triangleq f(x_k) - f(x^\star)$. This Lyapunov function yields the $O(L/k)$ convergence rate for the function value. For the squared gradient norm, however, this Lyapunov function can only exploit the $L$-smoothness property that transforms the function value to the gradient norm, giving the sub-optimal $O(L^2/k)$ rate, due to the absence of gradient information in this function. Our proof uses a different Lyapunov function: $\mathcal{E}(k) = ks \left( f(x_{k}) - f(x^{\star}) \right) + \frac{1}{2} \left\| x_{k} - x^{\star}   \right\|^{2}.$
See the proof of Theorem~\ref{thm: grad_descent_convex3} in Subsection~\ref{sec: discrete_gd_ex} for the full proof.


%to obtain a faster rate. The proof below highlights this point.





%Here, we point out that the traditional technique about gradient norm minimization of gradient flow takes the Lyapunov function
%\[
%\mathcal{E} = f(X) - f(x^\star),
%\] 
%and obtain by calculating time derivative  
%\[
%\min_{0 \leq u \leq t}  \left\| \nabla f(X(u)) \right\|^{2} \leq \frac{1}{t}.
%\]
%Based on the Lyapunov function constructed in~\cite{su2016differential}
%\[
%\mathcal{E} = t \left( f(X) - f(x^\star) \right) + \frac{1}{2} \left\| X - x^\star \right\|^{2},
%\]
%we can obtain 
%\[
%\min_{0 \leq u \leq t}  \left\| \nabla f(X(u)) \right\|^{2} \leq \frac{1}{t^2}.
%\]
%Rigorously and formally, it is shown in Theorem~\ref{thm: grad_flow_convex2} and its proof, which is deferred to Appendix~\ref{appendix: grad_flow}
%
%
%Starting the view of ODE, gradient flow~\eqref{eqn: grad_flow} is a  first-order ODE.\footnote{The concept of order of ODE is different from the order of information objective. The former is on the derivative of position of $x$ about $t$, such as $\dot{x}$, $\ddot{x}$, $\ldots$, while the latter is on the derivative of information objective $f(x)$ about $x$, such as $\nabla f(x)$, $\nabla^{2} f(x)$, $\ldots$.} The numerical scheme only contains two kinds, explicit scheme and implicit scheme. In this paper, we only discuss the simplest Euler scheme. 
%
%Apparently, the explicit Euler scheme of gradient flow is just the traditional gradient descent,  
%\begin{equation}
%\label{eqn: exp_grad}
%x_{k + 1} = x_{k} - s \nabla f(x_{k})
%\end{equation}
%with any initial $x_0 \in \mathbb{R}^n$. The theorems corresponding to the continuous version of gradient flow~\eqref{eqn: grad_flow} are shown in Appendix~\ref{sec: discrete_gd_ex}. In addition, the implicit Euler scheme of gradient flow (or implicit gradient descent) is  
%\begin{equation}
%\label{eqn: im_grad}
%x_{k + 1} = x_{k} - s \nabla f(x_{k + 1})
%\end{equation}
%with any initial $x_0 \in \mathbb{R}^n$. Although it is only practical for the implicit scheme in quadratic objective, there exists the theoretical meaning about studying it. The theorems corresponding to gradient flow~\eqref{eqn: grad_flow} are shown in Appendix~\ref{sec: discrete_gd_im}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

